Towards Guaranteed Safe AI: A Framework for Ensuring Robust and Reliable AI Systems

Ensuring that AI systems reliably and robustly avoid harmful or dangerous behaviours is a crucial challenge, especially for AI systems with a high degree of autonomy and general intelligence, or systems used in safety-critical contexts. In this paper, we will introduce and define a family of approaches to AI safety, which we will refer to as guaranteed safe (GS) AI. The core feature of these approaches is that they aim to produce AI systems which are equipped with high-assurance quantitative safety guarantees. This is achieved by the interplay of three core components: a world model (which provides a mathematical description of how the AI system affects the outside world), a safety specification (which is a mathematical description of what effects are acceptable), and a verifier (which provides an auditable proof certificate that the AI satisfies the safety specification relative to the world model). We outline a number of approaches for creating each of these three core components, describe the main technical challenges, and suggest a number of potential solutions to them. We also argue for the necessity of this approach to AI safety, and for the inadequacy of the main alternative approaches.

==> examples <==
\section{Examples of GS AI Solutions}\label{sec:examples}

This section we describe some concrete examples of practical problems and how they may be solved with a GS AI approach, which combine the different components described in the previous sections and fall along the different axes.

\begin{example}
Code Translation with LLMs.
\begin{itemize}
    \item Problem: Translate code in one programming language (e.g.\ C) to another (e.g.\ Rust) using AI systems (e.g.\ LLMs) with provable guarantees. 
    \item Specification: (i) Functional Correctness (source program is equivalent to target program with respect to relevant program state; (ii) Generated target code does not have specified classes of security vulnerabilities.
    \item World Model: (i) Constraints on the inputs to the program (pre-conditions), (ii) Threat models for security (what the attacker can/cannot do).
    \item AI System:  LLMs for Code Generation (e.g. models such as GPT-4, Claude, etc. or others expressly designed or fine-tuned for code generation).
    \item Kind of Guarantees: Formal proof of functional correctness and security (using a formal verification tool).
\end{itemize}
\end{example}

\begin{example}
Autonomous Vehicle (AV) Safety
\begin{enumerate}
    \item Problem: Design an AI-enabled autonomous driving system (ADS) that satisfies a formal specification of safety and functionality in specified scenarios, and also maintains a (smaller) core safety specification when outside those scenarios 
    \item Specification: A “rulebook”, a set of rules that have an associated pre-order, where each rule can be a specification written in a formalism that suits its purpose. Rules are mathematical objects that map behavioursbehaviors (or sets of behavioursbehaviors) to a value domain; they can be objective functions (cost/reward functions), temporal logic properties, probabilistic bound properties, automata, hyperproperties, etc. The overall specification would also include a “more restricted” specification that would be maintained by the backup system (of which there could be multiple levels).
    \item World Model: A set of scenarios in which the ADS operates that includes formal models of (i) the other components of the AV, (ii) agents and objects in the scenario, including their attributes and behaviourbehavior models, (iii) other attributes of the environment, such as spatial constraints of the physical world around the AV, time of day, weather conditions, etc., (iv) models of humans and their preferences and objectives. We expect these models will be stochastic in nature and some components of the world model will be learned from data/interactions while others will be encoded by domain experts or inferred/generated statically. Probabilistic programming languages (e.g. Scenic) offer one mechanism for world modellingmodeling for this application and have had some success in practice.  As in the case of the Specification, there would be world models also specified for the backup system(s) which constitute weaker assumptions about the operating environment.
    \item AI System: ADS integratesintegrate many types of AI/ML components with traditional hardware and software components. For example, deep neural networks are used in various steps of the autonomy pipeline including for perception, prediction, planning, and control. LLMs are being considered for use in interfaces to humans, to elicit preferences, explain the behaviourbehavior of AVs to occupants and others, etc. An ADS should also include runtime monitors that check whether the assumptions made in the world model (about the AV’s “operational design domain”) are maintained during operation, and, if not, to predictively take backup action.
    \item Kinds of Guarantees:  We expect most guarantees will be probabilistic in nature, especially because of the stochastic nature of the world model. These guarantees will be contingent on the distributional assumptions made in the world model.
\end{enumerate}
\end{example}

\begin{example}
Household Robots
\begin{enumerate}
    \item Problem: Provide assistance to humans in need of support at home.
    \item Specification: (i) Conduction of Diverse Household Tasks: Tasks include cleaning the room, organisingorganizing items, bringing items to humans, and navigating safely around people, ensuring no harm to humans. (ii) Adaptation to Human's Special Needs and Environment:  The robots should adapt to varying human needs and environments while grounding the original skills to the new conditions.
    \item World model: (i) Home Diversity: Various layouts of homes and diverse tasks for home management. (ii) Robot Constraints: Constraints governing the behaviourbehavior of the robots to ensure safety and efficiency.
    \item Learning Capability: The ability of robots to learn from interactions and adapt to new situations.
    \item AI System: VLMs equipped with multi-task learning capabilities and continuous learning mechanisms.
\end{enumerate}
\end{example}

\begin{example}
Medical diagnosis agent
\begin{enumerate}
    \item Problem: Facilitate disease diagnosis and provide medical advice.
    \item Specification: (i) Accurate Identification of Health Issues: Precisely diagnose healthcare concerns. (ii) Causal Understanding of Pathology: Provide insights into the underlying causes of the disease. (iii)Accurate Treatment: Offer precise and effective treatment recommendations.
    \item World Model: (i)Human Body: Understanding the complexities and nuances of human physiology and pathology. (ii) Environmental Factors: Consideration of external factors contributing to disease onset or progression.
    \item AI System: A multi-media input system capable of parsing diagnostic notes, interpreting medical imaging data, and delivering accurate diagnoses and treatment plans.
\end{enumerate}
\end{example}
